MP-Mat: A 3D-and-Instance-Aware Human Matting and Editing Framework with Multiplane Representation

Human instance matting aims to estimate an alpha matte for each human instance in an image, which is challenging as it easily fails in complex cases requiring disentangling mingled pixels belonging to multiple instances along hairy and thin boundary structures. In this work, we address this by introducing MP-Mat, a novel 3D-and-instance-aware matting framework with multiplane representation, where the multiplane concept is designed from two different perspectives: scene geometry level and instance level. Specifically, we first build feature-level multiplane representations to split the scene into multiple planes based on depth differences. This approach makes the scene representation 3D-aware, and can serve as an effective clue for splitting instances in different 3D positions, thereby improving interpretability and boundary handling ability especially in occlusion areas. Then, we introduce another multiplane representation that splits the scene in an instance-level perspective, and represents each instance with both matte and color. We also treat background as a special instance, which is often overlooked by existing methods. Such an instance-level representation facilitates both foreground and background content awareness, and is useful for other down-stream tasks like image editing. Once built, the representation can be reused to realize controllable instance-level image editing with high efficiency. Extensive experiments validate the clear advantage of MP-Mat in matting task. We also demonstrate its superiority in image editing tasks, an area under-explored by existing matting-focused methods, where our approach under zero-shot inference even outperforms trained specialized image editing techniques by large margins. Code is open-sourced at https://github.com/JiaoSiyi/MPMat.git}.

==> arg/removal.tex <==
\begin{algorithm}
\caption{Algorithm of Instance removal}
\textcolor[RGB]{128, 192, 128}{\# Inputs: original image (I), instances that require reordering (p, q)}

\textcolor[RGB]{128, 192, 128}{\# Outputs: new rendered image (O)}\\

\SetKwFunction{RegionFunction}{Removal\_region} 
\SetKwFunction{PlaneFunction}{Next\_plane}
\SetKwFunction{AsignFunction}{Asign}
\SetKwFunction{CompositeFunc}{Composite}
\SetKwFunction{RemovalFunc}{Removal}% 定义函数名称
\SetKwProg{Fn}{Function}{:}{} % 定义函数结构

\Fn{\RegionFunction{$R,index$}}{
    $M = \{(x, y) | R[index]['\alpha'](x, y) > 0\}$ \\
    \KwRet{$M$}
}
\Fn{\PlaneFunction{$R,index,position$}}{
    \For{$nextindex \leftarrow index+1$ \KwTo $len(R)-1$}{
    \If{$R[nextindex]['\alpha'][position]> 0$}{
            \KwRet{$nextindex$}
        }
}}
\Fn{\AsignFunction{$R,index,nextindex,position$}}{
   $R[nextindex]['\alpha'][position] += R[index]['\alpha'][position]$ \\
   \KwRet{$R$}
}
\Fn{\CompositeFunc{$R$}}{
    $O=0$\\
    \For{$index \leftarrow 0$ \KwTo $len(R)-1$}{
    $O = O+R[index]['\alpha']\cdot R[index]['c']$
}
    \KwRet{$O$}
}
\Fn{\RemovalFunc{$R,index$}}{
$M =$ \RegionFunction{$R,index$} \\
\For{$position \in M$}{
    $nextindex = $ \PlaneFunction{$R,index,position$}
    
$R = $ \AsignFunction{$R,index,nextindex,position$}

$O =$ \CompositeFunc{$R$}
}}
$R =$ MP-Mat($I$)\textcolor[RGB]{128, 192, 128}{\tcp{Instances are assigned indexes from small to large according to plane depth, with the largest index corresponding to the background}}

$O =$ \RemovalFunc{$R,j$}\tcp{late}
\end{algorithm}


==> table/ablation1.tex <==
\begin{table}[t]
  \begin{minipage}{0.48\linewidth}
    \centering
    \captionof{table}{Effects of the proposed SG-MP and \\Inst-MP in a global perspective.}
    \resizebox{0.8\linewidth}{!}{
        \begin{tabular}{cc|ll}
\hline
SG-MP        & Inst-MP      & \multicolumn{1}{c}{SAD} & \multicolumn{1}{c}{MSE} \\ \hline
             &              & 35.85                   & 0.87                  \\
             & $\checkmark$ & 33.78                   & 0.86                  \\
$\checkmark$ &              & 29.46                   & 0.60                  \\
$\checkmark$ & $\checkmark$ & \textbf{26.75}          & \textbf{0.49}         \\ \hline
\end{tabular}}
    \label{tab:ab}
  \end{minipage}
  \begin{minipage}{0.49\linewidth}
    \centering
    \captionof{table}{Components effects within SG-MP extraction.}
    \resizebox{0.75\linewidth}{!}{
    %\renewcommand{\arraystretch}{1.15} 
   \begin{tabular}{cc|ll}
\hline
Depth        & PGN          & \multicolumn{1}{c}{SAD} & \multicolumn{1}{c}{MSE} \\ \hline
             &              & 33.78                   & 0.86                  \\
$\checkmark$ &              & 31.82                   & 0.74                  \\
$\checkmark$ & $\checkmark$ & \textbf{26.75}          & \textbf{0.49}         \\ \hline
\end{tabular}}
\label{tab:sgmp}
  \end{minipage}
\end{table}

==> table/ablation2.tex <==
\begin{table}[t]
    \begin{minipage}{0.6\linewidth}
        \centering
        \captionof{table}{Component effect in Inst-MP extraction.}
        \resizebox{0.9\linewidth}{!}{
        \begin{tabular}{ccc|ll}
\hline
\begin{tabular}[c]{@{}c@{}}Background \\ Estimation\end{tabular} & \begin{tabular}[c]{@{}c@{}}Color \\ Estimation\end{tabular} & Refinement            & \multicolumn{1}{c}{SAD} & \multicolumn{1}{c}{MSE} \\ \hline
                                                                 & \multicolumn{1}{l}{}                                        &                       & 29.46                   & 0.60                  \\
$\checkmark$                                                     & \multicolumn{1}{l}{}                                        &                       & 28.53                   & 0.55                  \\
$\checkmark$                                                     & $\checkmark$                                                & \multicolumn{1}{l|}{} & 27.79                   & 0.52                  \\
$\checkmark$                                                     & $\checkmark$                                                & $\checkmark$          & \textbf{26.75}          & \textbf{0.49}         \\ \hline
\end{tabular}}
        \label{tab:instmp}
    \end{minipage}
    \begin{minipage}{0.38\linewidth}
        \centering
        \captionof{table}{Parameter analysis on $T$.}
        \resizebox{0.6\linewidth}{!}{
        \renewcommand{\arraystretch}{1.1} 
        \begin{tabular}{c|cc}
\hline
$T$ & SAD            & MSE           \\ \hline
0   & 27.79          & 0.52          \\
1   & 27.56          & 0.53          \\
10  & \textbf{26.75} & \textbf{0.49} \\
20  & 27.45          & 0.51          \\ \hline
\end{tabular}}
        \label{tab:T}
    \end{minipage}
\end{table}

==> table/experiments2.tex <==
\begin{table}[]
    %\vspace{-24pt}
    \centering
    \captionof{table}{Component effect in Inst-MP extraction.}
    \resizebox{0.76\linewidth}{!}{ 
    \begin{tabular}{ccc|ll}
\hline
Background Estimation & Color Estimation     & Refinement            & \multicolumn{1}{c}{SAD} & \multicolumn{1}{c}{MSE} \\ \hline
                      & \multicolumn{1}{l}{} &                       & 29.46                   & 0.0060                  \\
$\checkmark$          & \multicolumn{1}{l}{} &                       & 28.53                   & 0.0055                  \\
$\checkmark$          & $\checkmark$         & \multicolumn{1}{l|}{} & 27.79                   & 0.0052                  \\
$\checkmark$          & $\checkmark$         & $\checkmark$          & \textbf{26.75}          & \textbf{0.0049}         \\ \hline
\end{tabular}}
        \label{tab:instmp}
\end{table}

==> table/experiments3.tex <==
\begin{table}[]
    \begin{minipage}{\textwidth}
        \centering
\caption{Quantitative comparison on instance removal. BI refers to an off-the-shelf background inpainting method used to enhance the inpainting of the corresponding region.}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|ccc|clc}
\hline
Editing Method   & Mean L1 Loss (\downarrow) & Mean L2 Loss (\downarrow) & PSNR (\uparrow) & \multicolumn{3}{c}{Time per editing}                                       \\ \hline
Inst-inpaint     & 12.69\%                                  & 2.58\%                                   & 23.09db                        & \multicolumn{3}{c}{0.1982}                                                 \\
Dragon Diffusion & 12.13\%                                  & 2.49\%                                   & 22.17db                        & \multicolumn{3}{c}{0.2139}                                                 \\ \hline
Matting Method   & Mean L1 Loss (\downarrow) & Mean L1 Loss (\downarrow) & PSNR (\uparrow) & \multicolumn{2}{l}{time per image}  & \multicolumn{1}{l}{time per editing} \\ \hline
MaGGie      & 11.39\%                                  & 2.13\%                                   & 20.77db                        & \multicolumn{2}{c}{0.2369}          & \multirow{4}{*}{0.0003}               \\
Ours       &  9.37\%                                   & 1.96\%                                   & 23.58db                        & \multicolumn{2}{c}{0.1434}          &                                      \\
MaGGie (w/ BI)      & 5.49\%                                   & 0.87\%                                   & 21.42db                        & \multicolumn{2}{c}{0.1951}          &                                      \\
Ours (w/ BI)        & \textbf{3.73\%}                          & \textbf{0.84\%}                          & \textbf{25.79db}               & \multicolumn{2}{c}{\textbf{0.1117}} &                                      \\ \hline
\end{tabular}}
\label{tab:removal}
        
    \end{minipage}
    \begin{minipage}{\textwidth}
        \small 
\centering
\vspace{12pt}
\caption{Quantitative comparison on occlusion reordering.}
\begin{tabular}{c|ccc|c}
\hline
Method           & Mean L1 Loss (\downarrow)    & Mean L2 Loss (\downarrow)    & PSNR (\uparrow)             & Speed           \\ \hline
Inst-inpaint     & 12.65\%         & 3.42\%          & 21.2db           & 0.2547          \\
Dragon Diffusion & 13.85\%         & 3.66\%          & 19.82db          & 0.2849          \\ \hline
MaGGle           & 4.79\%          & 0.84\%          & 25.76db          & 0.1823          \\
ours             & \textbf{3.26\%} & \textbf{0.79\%} & \textbf{28.32db} & \textbf{0.1739} \\ \hline
\end{tabular}
\label{tab:reordering}
    \end{minipage}
\end{table}

==> table/fps.tex <==
\begin{table}[]
     \centering
    \caption{Quantitative comparison on single-instance datasets.}

    \resizebox{0.85\linewidth}{!}{
   \begin{tabular}{lc|cccc}
\hline
\multicolumn{2}{c|}{\multirow{3}{*}{Method}}                            & \multicolumn{4}{c}{Datasets}                                                           \\ \cline{3-6} 
\multicolumn{2}{c|}{}                                                   & \multicolumn{2}{c|}{P3M-500-P}                       & \multicolumn{2}{c}{P3M-500-NP}  \\
\multicolumn{2}{c|}{}                                                   & SAD           & \multicolumn{1}{c|}{MSE}             & SAD           & MSE             \\ \hline
\multicolumn{1}{l|}{\multirow{3}{*}{instance-agnostic}} & LF            & 42.95         & \multicolumn{1}{c|}{0.0191}          & 32.59         & 0.0131          \\
\multicolumn{1}{l|}{}                                   & P3MNet        & 8.73          & \multicolumn{1}{c|}{0.0026}          & 11.23         & 0.0035          \\
\multicolumn{1}{l|}{}                                   & GFM           & 13.20         & \multicolumn{1}{c|}{0.0050}          & 15.50         & 0.0056          \\ \hline
\multicolumn{1}{l|}{\multirow{4}{*}{instance-aware}}    & InstMatte     & 12.49         & \multicolumn{1}{c|}{0.0048}          & 16.71         & 0.0057          \\
\multicolumn{1}{l|}{}                                   & E2E-HIM       & 7.96          & \multicolumn{1}{c|}{0.0024}          & 9.25          & 0.0030          \\
\multicolumn{1}{l|}{}                                   & Maggie        & 8.94          & \multicolumn{1}{c|}{0.0030}          & 11.39         & 0.0037          \\
\multicolumn{1}{l|}{}                                   & MP-Mat (Ours) & \textbf{6.88} & \multicolumn{1}{c|}{\textbf{0.0022}} & \textbf{8.37} & \textbf{0.0028} \\ \hline
\end{tabular}}
\label{tab:single_comp}
\end{table}

==> table/multi_comp.tex <==
\begin{table}[]
\centering
\caption{Quantitative comparison on multi-instance datasets.}
\resizebox{0.6\linewidth}{!}{
\begin{tabular}{lcccc}
\hline
\multicolumn{1}{l|}{\multirow{3}{*}{Method}} & \multicolumn{4}{c}{Dataset}                                                                         \\ \cline{2-5} 
\multicolumn{1}{l|}{}                        & \multicolumn{2}{c|}{HIM-100k}                                    & \multicolumn{2}{c}{SMPMat}       \\
\multicolumn{1}{l|}{}                        & SAD                       & \multicolumn{1}{c|}{MSE}             & SAD            & MSE             \\ \hline
\multicolumn{5}{l}{\textit{\textbf{Instance-agnostic}}}                                                                                                              \\ \hline
\multicolumn{1}{l|}{FBA(+Mask RCNN)}         & \multicolumn{1}{l}{38.25} & \multicolumn{1}{c|}{0.0095}          & 42.36          & 0.1120           \\
\multicolumn{1}{l|}{FBA(+SOLO)}              & 38.18                     & \multicolumn{1}{c|}{0.0094}          & 41.23          & 0.0096          \\
\multicolumn{1}{l|}{FBA(+EVA)}               & 37.76                     & \multicolumn{1}{c|}{0.0091}          & 39.82          & 0.0095          \\
\multicolumn{1}{l|}{MG(+Mask RCNN)}          & 40.51                     & \multicolumn{1}{c|}{0.0097}          & 41.58          & 0.106           \\
\multicolumn{1}{l|}{MG(+SOLO)}               & 39.26                     & \multicolumn{1}{c|}{0.0095}          & 40.79          & 0.0095          \\
\multicolumn{1}{l|}{MG(+EVA)}                & 38.19                     & \multicolumn{1}{c|}{0.0094}          & 39.73          & 0.0095          \\ \hline
\multicolumn{5}{l}{\textit{\textbf{Instance-agnostic}}}                                                                                                              \\ \hline
\multicolumn{1}{l|}{InstMatte}               & 37.34                     & \multicolumn{1}{c|}{0.0093}          & 40.19          & 0.0096          \\
\multicolumn{1}{l|}{E2E-HIM}                 & 32.22                     & \multicolumn{1}{c|}{0.0084}          & 38.55          & 0.0093          \\
\multicolumn{1}{l|}{Maggie}                  & 29.18                     & \multicolumn{1}{c|}{0.0077}          & 36.72          & 0.0090          \\
\rowcolor[HTML]{C0C0C0} 
\multicolumn{1}{l|}{\cellcolor[HTML]{C0C0C0}MP-Mat (Ours)} & \textbf{26.75}            & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}\textbf{0.0069}} & \textbf{33.25} & \textbf{0.0081}              \\ \hline
\end{tabular}}
\label{tab:multi_comp}
\end{table}



==> table/object_change.tex <==
\begin{table}[]
% \scriptsize
\footnotesize
\centering
\caption{Quantitative comparison on occlusion reordering.}
\begin{tabular}{c|ccc|c}
\hline
Method           & Mean L1 Loss (\downarrow)    & Mean L2 Loss (\downarrow)    & PSNR (\uparrow)             & Speed           \\ \hline
Inst-inpaint     & 12.65\%         & 3.42\%          & 21.2db           & 0.2547          \\
Dragon Diffusion & 13.85\%         & 3.66\%          & 19.82db          & 0.2849          \\ \hline
MaGGle           & 4.79\%          & 0.84\%          & 25.76db          & 0.1823          \\
ours             & \textbf{3.26\%} & \textbf{0.79\%} & \textbf{28.32db} & \textbf{0.1739} \\ \hline
\end{tabular}
\label{tab:reordering}
\end{table}

==> table/object_remove.tex <==
\begin{table}[]
\centering
\caption{Quantitative comparison on instance removal. BI refers to an off-the-shelf background inpainting method used to enhance the inpainting of the corresponding region.}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|ccc|clc}
\hline
Editing Method   & Mean L1 Loss (\downarrow) & Mean L2 Loss (\downarrow) & PSNR (\uparrow) & \multicolumn{3}{c}{Time per editing}                                       \\ \hline
Inst-inpaint     & 12.69\%                                  & 2.58\%                                   & 23.09db                        & \multicolumn{3}{c}{0.1982}                                                 \\
Dragon Diffusion & 12.13\%                                  & 2.49\%                                   & 22.17db                        & \multicolumn{3}{c}{0.2139}                                                 \\ \hline
Matting Method   & Mean L1 Loss (\downarrow) & Mean L1 Loss (\downarrow) & PSNR (\uparrow) & \multicolumn{2}{l}{time per image}  & \multicolumn{1}{l}{time per editing} \\ \hline
MaGGie      & 11.39\%                                  & 2.13\%                                   & 20.77db                        & \multicolumn{2}{c}{0.1497}          & \multirow{4}{*}{0.012}               \\
Ours       &  9.37\%                                   & 1.96\%                                   & 23.58db                        & \multicolumn{2}{c}{0.1434}          &                                      \\
MaGGie (w/ BI)      & 5.49\%                                   & 0.87\%                                   & 21.42db                        & \multicolumn{2}{c}{0.1199}          &                                      \\
Ours (w/ BI)        & \textbf{3.73\%}                          & \textbf{0.84\%}                          & \textbf{25.79db}               & \multicolumn{2}{c}{\textbf{0.1117}} &                                      \\ \hline
\end{tabular}}
\label{tab:removal}
\end{table}

==> table/plane_num.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\begin{tabular}{c|c|c|cccc}
\hline
\multirow{2}{*}{Method}    & \multirow{2}{*}{Instance Segmentor} & Instance Segmentation on COCO & \multicolumn{4}{c}{Instance Matting on HIM-100K} \\
                           &                                     & Mask AP                       & SAD↓      & MSE↓     & Params↓     & Speed↓      \\ \hline
\multirow{6}{*}{InstMatte} & MaskRCNN (ICCV'17)                  & 42.5                          & 37.34     & 0.93     & 14.57M      & 46.41ms     \\
                           & EVA (CVPR'23)                       & 55.0                          & 35.49     & 0.85     & 1074M       & 184.39ms    \\
                           & CBNet (GitHub'24)                   & 56.1                          & 35.17     & 0.84     & 674M        & 153.85ms    \\
                           & Mix result                          & 52.4                          & 35.52     & 0.87     & -           & -           \\
                           & Mean                                & -                             & 35.88     & 0.87     & -           & -           \\
                           & Std                                 & -                             & 0.85      & 0.03     & -           & -           \\ \hline
\multirow{5}{*}{Maggie}    & MaskRCNN (ICCV'17)                  & 42.5                          & 29.48     & 0.78     & 14.57M      & 46.41ms     \\
                           & EVA (CVPR'23)                       & 55.0                          & 28.73     & 0.75     & 1074M       & 184.39ms    \\
                           & CBNet (GitHub'24)                   & 56.1                          & 28.55     & 0.75     & 674M        & 153.85ms    \\
                           & Mean                                & -                             & 28.88     & 0.76     & -           & -           \\
                           & Std                                 & -                             & 0.36      & 0.01     & -           & -           \\ \hline
\end{tabular}
\end{table}





==> table/single_comp.tex <==
\begin{table}[]
     \centering
    \caption{Quantitative comparison on single-instance datasets.}

    \resizebox{0.85\linewidth}{!}{
   \begin{tabular}{lc|cccc}
\hline
\multicolumn{2}{c|}{\multirow{3}{*}{Method}}                            & \multicolumn{4}{c}{Datasets}                                                           \\ \cline{3-6} 
\multicolumn{2}{c|}{}                                                   & \multicolumn{2}{c|}{P3M-500-P}                       & \multicolumn{2}{c}{P3M-500-NP}  \\
\multicolumn{2}{c|}{}                                                   & SAD           & \multicolumn{1}{c|}{MSE}             & SAD           & MSE             \\ \hline
\multicolumn{1}{l|}{\multirow{3}{*}{instance-agnostic}} & LF            & 42.95         & \multicolumn{1}{c|}{0.0191}          & 32.59         & 0.0131          \\
\multicolumn{1}{l|}{}                                   & P3MNet        & 8.73          & \multicolumn{1}{c|}{0.0026}          & 11.23         & 0.0035          \\
\multicolumn{1}{l|}{}                                   & GFM           & 13.20         & \multicolumn{1}{c|}{0.0050}          & 15.50         & 0.0056          \\ \hline
\multicolumn{1}{l|}{\multirow{4}{*}{instance-aware}}    & InstMatte     & 12.49         & \multicolumn{1}{c|}{0.0048}          & 16.71         & 0.0057          \\
\multicolumn{1}{l|}{}                                   & E2E-HIM       & 7.96          & \multicolumn{1}{c|}{0.0024}          & 9.25          & 0.0030          \\
\multicolumn{1}{l|}{}                                   & Maggie        & 8.94          & \multicolumn{1}{c|}{0.0030}          & 11.39         & 0.0037          \\
\multicolumn{1}{l|}{}                                   & MP-Mat (Ours) & \textbf{6.88} & \multicolumn{1}{c|}{\textbf{0.0022}} & \textbf{8.37} & \textbf{0.0028} \\ \hline
\end{tabular}}
\label{tab:single_comp}
\end{table}
